MORAD: Reinforcement Learning with Multi-Objective Rewards for RNA Inverse Design

We introduce MORAD, an online reinforcement learning framework for backbone-conditioned RNA diffusion models that trains a single shared policy across diverse target backbones. Structure-conditioned RNA inverse design seeks nucleotide sequences compatible with a target three-dimensional backbone, yet existing reinforcement learning approaches either optimize a separate policy for each target backbone or rely on offline preference optimization, leaving online post-training of a reusable backbone-conditioned model largely unexplored. MORAD combines backbone-conditioned group sampling, group-relative reward normalization, and a forward-process diffusion objective. Beyond existing RL rewards that primarily target tertiary structural quality, MORAD jointly optimizes six measurements spanning tertiary geometry, base pairing, ensemble behavior, and sequence composition. To aggregate these heterogeneous objectives despite differences in scale and optimization direction, MORAD maps each measurement to a bounded desirability score and combines them with a weighted geometric mean. Compared with a tertiary-structure-only reward, this multi-objective formulation improves 10 of the 11 evaluation metrics that have a preferred direction. Applied to pretrained RIDE, MORAD improves GDT-TS by 16.0% (from 0.3300 to 0.3827) and pairing MCC by 19.4% (from 0.6110 to 0.7295), while reducing normalized ensemble defect by 27.5% (from 0.3906 to 0.2830). On the test set, MORAD outperforms RiboDiffusion, gRNAde, and RDesign across tertiary structural accuracy, secondary-structure pairing, and thermodynamic quality, establishing a new state of the art in structure-conditioned RNA inverse design.

==> table_checkpoints.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrr@{}}
\toprule
Checkpoint & GDT-TS $\uparrow$ & TM(C4$\prime$) $\uparrow$ & RMSD (\AA) $\downarrow$ & C1$\prime$ TM $\uparrow$ & Recovery $\uparrow$ \\
\midrule
Step 180 & \shortstack{0.3682\\$\pm$0.0177} & \shortstack{0.3218\\$\pm$0.0198} & \shortstack{8.263\\$\pm$0.490} & \shortstack{0.3716\\$\pm$0.0171} & \shortstack{0.5074\\$\pm$0.0108} \\
Step 230 & \shortstack{0.3617\\$\pm$0.0184} & \shortstack{0.3208\\$\pm$0.0201} & \shortstack{8.733\\$\pm$0.554} & \shortstack{0.3697\\$\pm$0.0176} & \shortstack{0.5021\\$\pm$0.0107} \\
Step 340 & \shortstack{0.3686\\$\pm$0.0185} & \shortstack{0.3271\\$\pm$0.0205} & \shortstack{8.435\\$\pm$0.530} & \shortstack{0.3771\\$\pm$0.0177} & \shortstack{0.5032\\$\pm$0.0104} \\
\textbf{MORAD (390)} & \shortstack{0.3774\\$\pm$0.0179} & \shortstack{0.3338\\$\pm$0.0202} & \shortstack{7.981\\$\pm$0.489} & \shortstack{0.3833\\$\pm$0.0177} & \shortstack{0.5102\\$\pm$0.0106} \\
\bottomrule
\end{tabular*}


==> table_reward_control.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrr@{}}
\toprule
Measurement & RIDE & + Structural reward & + MORAD reward \\
\midrule
\multicolumn{4}{@{}l}{\itshape Tertiary structure} \\
\quad GDT-TS $\uparrow$ & 0.3300 & 0.3627 & \textbf{0.3694} \\
\quad TM-score $\uparrow$ & 0.2841 & 0.3194 & \textbf{0.3358} \\
\quad RMSD (\AA) $\downarrow$ & 9.720 & 8.369 & \textbf{8.207} \\
\quad C1$\prime$ TM $\uparrow$ & 0.3538 & 0.3818 & \textbf{0.3919} \\
\addlinespace[2pt]
\multicolumn{4}{@{}l}{\itshape Secondary structure and recovery} \\
\quad MCC $\uparrow$ & 0.6208 & 0.6612 & \textbf{0.6978} \\
\quad F1 $\uparrow$ & 0.6103 & 0.6568 & \textbf{0.6901} \\
\quad ED (nt) $\downarrow$ & 29.08 & 26.85 & \textbf{24.27} \\
\quad ED/nt $\downarrow$ & 0.3872 & 0.3569 & \textbf{0.3256} \\
\quad Recovery $\uparrow$ & 0.5033 & 0.5097 & \textbf{0.5124} \\
\addlinespace[2pt]
\multicolumn{4}{@{}l}{\itshape Equilibrium ensemble} \\
\quad $H_{\rm pair}$ $\downarrow$ & 0.3249 & 0.2851 & \textbf{0.2800} \\
\quad $p_{\rm MFE}$ $\uparrow$ & 0.3281 & \textbf{0.3880} & 0.3847 \\
\quad MFE (kcal/mol) & -23.77 & -29.81 & -26.49 \\
\quad GC fraction & 0.5304 & 0.5912 & 0.4970 \\
\addlinespace[2pt]
\multicolumn{4}{@{}l}{\itshape Candidate diversity} \\
\quad Hamming & 0.2971 & 0.2224 & 0.2607 \\
\bottomrule
\end{tabular*}


==> table_secondary.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Model & Precision $\uparrow$ & Recall $\uparrow$ & F1 $\uparrow$ & MCC $\uparrow$ \\
\midrule
RiboDiffusion & 0.3563 & 0.3074 & 0.3212 & 0.3267 \\
gRNAde ($T=0.1$) & 0.7276 & 0.6099 & 0.6482 & 0.6734 \\
RDesign & 0.7084 & 0.6110 & 0.6462 & 0.6566 \\
\midrule
RIDE & 0.6472 & 0.5717 & 0.5939 & 0.6110 \\
\textbf{MORAD} & \textbf{0.7824} & \textbf{0.6816} & \textbf{0.7226} & \textbf{0.7295} \\
\bottomrule
\end{tabular*}


==> table_secondary_counts.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Model & $n$(Precision) & $n$(Recall) & $n$(F1) & $n$(MCC) \\
\midrule
RiboDiffusion & 133 & 137 & 137 & 133 \\
gRNAde ($T=0.1$) & 132 & 137 & 137 & 132 \\
RDesign & 135 & 137 & 137 & 135 \\
\midrule
RIDE & 133 & 137 & 137 & 133 \\
\textbf{MORAD} & 136 & 137 & 137 & 136 \\
\bottomrule
\end{tabular*}


==> table_sequence_diversity.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Model & Hamming diversity $\uparrow$ & 3-mer diversity $\uparrow$ & Targets & Candidates \\
\midrule
RiboDiffusion & 0.2744 & 0.3964 & 153 & 1224 \\
gRNAde ($T=0.1$) & 0.1579 & 0.2406 & 153 & 1224 \\
RDesign & \textbf{0.4368} & \textbf{0.6184} & 153 & 1224 \\
\midrule
RIDE & 0.2971 & 0.5270 & 153 & 1224 \\
\textbf{MORAD} & 0.2344 & 0.3673 & 153 & 1224 \\
\bottomrule
\end{tabular*}


==> table_tertiary.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrrrr@{}}
\toprule
Model & \shortstack{GDT-TS\\$\uparrow$} & \shortstack{TM(C4$\prime$)\\$\uparrow$} & \shortstack{RMSD (\AA)\\$\downarrow$} & \shortstack{TM(C1$\prime$)\\$\uparrow$} & \shortstack{Success\\$\uparrow$} & \shortstack{Recovery\\$\uparrow$} & \shortstack{lDDT(C4$\prime$)\\$\uparrow$} & \shortstack{pLDDT\\$\uparrow$} & \shortstack{Coarse clash\\$\downarrow$} \\
\midrule
RiboDiffusion & 0.3132 & 0.2839 & 10.9215 & 0.3613 & 0.2549 & \textbf{0.5165} & 0.6174 & \textbf{0.6937} & 73.5383 \\
gRNAde ($T=0.1$) & 0.3591 & 0.3179 & 8.8374 & 0.3642 & 0.2484 & 0.5115 & 0.6607 & 0.6482 & 23.7261 \\
RDesign & 0.3291 & 0.2902 & 10.3441 & 0.3392 & 0.2549 & 0.4720 & 0.6368 & 0.6202 & 40.4457 \\
\midrule
RIDE & 0.3300 & 0.2841 & 9.7199 & 0.3538 & 0.2484 & 0.5039 & 0.6622 & 0.6671 & 22.7503 \\
\textbf{MORAD} & \textbf{0.3827} & \textbf{0.3400} & \textbf{7.9196} & \textbf{0.3855} & \textbf{0.3007} & 0.5056 & \textbf{0.6774} & 0.6726 & \textbf{11.9438} \\
\bottomrule
\end{tabular*}


==> table_thermodynamics.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrr@{}}
\toprule
Model & MFE $\sim$ & EFE $\sim$ & NED $\downarrow$ & PE $\downarrow$ & MFEfreq $\uparrow$ \\
\midrule
RiboDiffusion & -21.716 & -22.847 & 0.6056 & 0.4284 & 0.2980 \\
gRNAde ($T=0.1$) & -28.092 & -28.918 & 0.3458 & 0.2652 & 0.4289 \\
gRNAde ($T=0.8$) & -25.186 & -26.212 & 0.3830 & 0.3260 & 0.3266 \\
RDesign & -28.863 & -29.708 & 0.3349 & 0.2775 & 0.3961 \\
\midrule
RIDE & -23.614 & -24.643 & 0.3906 & 0.3059 & 0.3350 \\
\textbf{MORAD} & -30.149 & -30.937 & \textbf{0.2830} & \textbf{0.2102} & \textbf{0.4402} \\
\bottomrule
\end{tabular*}


==> table_thermodynamics_full.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrr@{}}
\toprule
Metric & \shortstack{Ribo\\Diffusion} & \shortstack{gRNAde\\$T=0.1$} & \shortstack{gRNAde\\$T=0.8$} & RDesign & RIDE & MORAD & Native \\
\midrule
MFE $\sim$ & -21.716 & -28.092 & -25.186 & -28.863 & -23.614 & -30.149 & -21.261 \\
EFE $\sim$ & -22.847 & -28.918 & -26.212 & -29.708 & -24.643 & -30.937 & --- \\
ED $\downarrow$ & 43.653 & 26.913 & 28.486 & 25.502 & 29.184 & \textbf{21.403} & 28.049 \\
NED $\downarrow$ & 0.6056 & 0.3458 & 0.3830 & 0.3349 & 0.3906 & \textbf{0.2830} & 0.3741 \\
EDiv $\sim$ & 10.427 & 7.471 & 8.252 & 7.187 & 7.512 & 5.605 & 8.685 \\
PE $\downarrow$ & 0.4284 & 0.2652 & 0.3260 & 0.2775 & 0.3059 & \textbf{0.2102} & 0.3581 \\
MFEfreq $\uparrow$ & 0.2980 & 0.4289 & 0.3266 & 0.3961 & 0.3350 & \textbf{0.4402} & 0.3119 \\
$T_m$ $\sim$ & 73.91 & 73.07 & 73.57 & 71.71 & 72.54 & 72.52 & --- \\
GC $\sim$ & 0.5734 & 0.5529 & 0.5650 & 0.5195 & 0.5400 & 0.5393 & --- \\
\bottomrule
\end{tabular*}

